On $C^0$-persistent homology and trees

In this paper we give a metric construction of a tree which correctly identifies connected components of superlevel sets of $\mathbb{R}$-valued continuous functions $f$ on $X$ and show that it is possible to retrieve the $H_0$-persistent diagram from this tree. We revisit the notion of homological dimension previously introduced by Schweinhart and give some bounds for the latter in terms of the upper-box dimension of $X$, thereby partially answering a question of the same author. We prove a quantitative version of the Wasserstein stability theorem valid for regular enough $X$ and $\alpha$-H\"older functions and discuss some applications of this theory to random fields and the topology of their superlevel sets.

==> C0-Homology 2/commands.tex <==
%% numbering
\newcommand{\Eqr}[1]{(\ref{#1})}
\newcommand{\mysection}[1]{\setcounter{equation}{0}\section{#1}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}

%% colors
\definecolor{lightgrey}{gray}{0.9}

%unit of length (for drawing Feynman diagrams)
\setlength{\unitlength}{1mm}

% lazy to type
\newcommand{\etal}{\textit{et al.}}

%Probability theory
\newcommand{\expect}[1]{\mathbb{E} \!\left [ #1\right]}
\newcommand{\cexpect}[2]{\mathbb{E} \!\left[ #1 \, \middle\vert \, #2 \right]}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\ora}{\overrightarrow}
\newcommand{\ola}{\overleftarrow}

\newcommand{\innermid}{\nonscript\;\delimsize\vert\nonscript\;}
\newcommand{\activatebar}{%
  \begingroup\lccode`\~=`\|
  \lowercase{\endgroup\let~}\innermid 
  \mathcode`|=\string"8000
}


\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}


%Ensembles
\newcommand{\II}{\mathcal{I}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\Sphere}{\mathbb{S}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\Euc}{\mathbb{E}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\Cl}{\mathcal{C}\ell}
\newcommand{\catC}{\mathcal{C}}
\newcommand{\catA}{\mathcal{A}}
\newcommand{\bcode}{\mathcal{B}}
\newcommand{\ModA}{\textbf{Mod}_A}
\newcommand{\FreeA}{\textbf{Free}_A}
\newcommand{\Top}{\textbf{Top}}
\newcommand{\Set}{\textbf{Set}}
\newcommand{\Poset}{\textbf{Poset}}
\newcommand{\Deltaop}{\Delta^{\text{op}}}
\newcommand{\Vectk}{\textbf{Vect}_k}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\vC}{\v{C}}
\newcommand{\wfs}{\text{wfs}}
\newcommand{\Linfty}{L^{\infty}}
\newcommand{\pvar}{p-\text{var}}
\newcommand{\Var}{\text{Var}}
\newcommand{\suchthat}{\;\ifnum\currentgrouptype=16 \middle\fi|\;}

%Measure theory and operators
\DeclareMathOperator\supp{supp}
\DeclareMathOperator\csch{csch}
\DeclareMathOperator\sech{sech}
\DeclareMathOperator\id{id}
\DeclareMathOperator\Vol{Vol}
\DeclareMathOperator\homdim{H-dim}
\DeclareMathOperator\thomdim{TH-dim}

%Special functions
\DeclareMathOperator\erfc{erfc}
\DeclareMathOperator\PH{PH}
\DeclareMathOperator\Pers{Pers}
\DeclareMathOperator\erf{erf}
\DeclareMathOperator\erfi{erfi}
\DeclareMathOperator\Hom{Hom}
\DeclareMathOperator\End{End}
\DeclareMathOperator\Stab{Stab}
\DeclareMathOperator\Orb{Orb}
\DeclareMathOperator\sgn{sgn}
\DeclareMathOperator\Ad{Ad}
\DeclareMathOperator\ad{ad}
\DeclareMathOperator\Aut{Aut}
\DeclareMathOperator\Tor{Tor}
\DeclareMathOperator\Ext{Ext}
\DeclareMathOperator\Homeo{Homeo}
\DeclareMathOperator\vol{vol}
\DeclareMathOperator\Hess{Hess}
\DeclareMathOperator\Lip{Lip}
\DeclareMathOperator\Hol{Hol}
\DeclareMathOperator\Tr{Tr}
\DeclareMathOperator\Image{Im}
\DeclareMathOperator\coker{coker}
\DeclareMathOperator\rk{rank}
\DeclareMathOperator\dgm{dgm}
\DeclareMathOperator\Dgm{Dgm}
\DeclareMathOperator\Ind{Ind}
\DeclareMathOperator\Crit{Crit}
\DeclareMathOperator\Real{Re}
\DeclareMathOperator\Imag{Im}
\DeclareMathOperator\Ai{Ai}
\DeclareMathOperator\Bi{Bi}
\DeclareMathOperator\Alg{Alg}
\DeclareMathOperator\OT{OT}
\DeclareMathOperator\updim{\overline{dim}}
\DeclareMathOperator\downdim{\underline{dim}}
\DeclareMathOperator\Li{Li}
\DeclareMathOperator\Res{Res}
\DeclareMathOperator\Herm{He}




%Lie Algebras
\newcommand{\g}{\mathfrak{g}}
\newcommand{\h}{\mathfrak{h}}
\newcommand{\mfkk}{\mathfrak{k}}
\newcommand{\p}{\mathfrak{p}}
\newcommand{\gl}{\mathfrak{gl}}
\newcommand{\sln}{\mathfrak{sl}}
\newcommand{\su}{\mathfrak{su}}
\newcommand{\so}{\mathfrak{so}}
\newcommand{\spn}{\mathfrak{sp}}
\newcommand{\isom}{\mathfrak{iso}}
\newcommand{\spin}{\mathfrak{spin}}
\newcommand{\W}{\mathfrak{W}}


%\newcommand{\deg}{\text{deg}}
\newcommand{\eqand}{\quad \text{ and } \quad}
\newcommand{\eqor}{\quad \text{ or } \quad}

\newcommand{\tX}{\tilde{X}}
\newcommand{\tY}{\tilde{Y}}



%Linear ebra
\newcommand{\B}{\langle }
\newcommand{\K}{\rangle }
\newcommand{\tensor}{\otimes}
\newcommand{\ds}{\oplus}
\newcommand{\DS}{\bigoplus}
%\newcommand{\updim}{\overline{\dim}}
\newcommand{\normal}{\trianglelefteq}
\newcommand{\iso}{\cong}



%Greek
\newcommand{\al}{\alpha}
\newcommand{\eps}{\epsilon}
\newcommand{\lab}{\label}
\newcommand{\om}{\omega}
\newcommand{\veps}{\varepsilon}
\newcommand{\vp}{\varphi}

%Weinberg Angles
\newcommand{\stw}{\sin \theta_W}
\newcommand{\ctw}{\cos \theta_W}

%Math mode and other
\newcommand{\bd}{\begin{displaymath}
\begin{tikzcd}}
\newcommand{\ed}{\end{tikzcd}
\end{displaymath}}
\newcommand{\bmat}{\begin{pmatrix}}
\newcommand{\emat}{\end{pmatrix}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\btikz}{\begin{tikzcd}}
\newcommand{\etikz}{\end{tikzcd}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
%\newcommand{\ss}{\smallskip}
\newcommand{\ms}{\medskip}
\newcommand{\bs}{\bigskip}
\newcommand{\pb}{\pagebreak}
%\newcommand{\ni}{\noindent}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\ov}{\over}
\newcommand{\nonum}{\nonumber}
\newcommand{\up}{\uparrow}
\newcommand{\dn}{\downarrow}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\bra}{\langle}
\newcommand{\ket}{\rangle}
\newcommand{\XX}{\mathcal{X}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


%Analysis
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

%Constants and math symbols and integrals
\newcommand{\Gammabar}{{\bar\Gamma}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\KK}{\mathcal{K}}
%\newcommand{\iff}{\; \Longleftrightarrow \;}
\newcommand{\E}{{\rm e}}
\newcommand{\I}{{\rm i}}
\newcommand{\M}{{\rm m}}
\newcommand{\D}{{\rm d}}
\newcommand{\Ord}{{\rm O}}
\newcommand{\del}{\partial}
\newcommand{\IH}{\I\hbar}
\newcommand{\Equiv}{\hspace{10pt}\Longleftrightarrow\hspace{10pt}}
\newcommand{\xx}{{\bf{x}}}
\newcommand{\zz}{{\bf{z}}}
\newcommand{\yy}{{\bf{y}}}
\newcommand{\kk}{{\bf{k}}}
\newcommand{\qq}{{\bf{q}}}
\newcommand{\pp}{{\bf{p}}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\intddx}{\int {\rm d}^D {\bf x} \,}
\newcommand{\intdphi}{\int \mathcal{D}\phi \,}
\newcommand{\intdpphi}{\int \mathcal{D}' \phi \,}
\newcommand{\intddk}{\int \frac{{\rm d}^D {\bf k}}{(2\pi)^D} \,}
\newcommand{\intdnx}{\int_{\R^n} {\rm d}^n \xx \,\,}
%Long comment
\newcommand{\comment}[1]{}


%Latin abbreviations
\newcommand{\etc}{{\it etc. }}
\newcommand{\ie}{{\it i.e. }}
\newcommand{\cf}{{\it cf. }}
\newcommand{\eg}{{\it e.g. }}

%Barred symbols
\newcommand{\mubar}{{\bar \mu}}
\newcommand{\delbar}{{\bar \del}}
\newcommand{\ebar}{{\bar \e}}
\newcommand{\Qbar}{{\bar Q}}
\newcommand{\Dbar}{{\bar D}}
\newcommand{\Wbar}{{\overline W}}
\newcommand{\sibar}{{\bar\sigma}} 
\newcommand{\chibar}{{\bar\chi}} 
\newcommand{\xibar}{{\bar\xi}} 
\newcommand{\psibar}{{\bar\psi}} 
\newcommand{\Phibar}{{\bar\Phi}} 
\newcommand{\Psibar}{{\bar\Psi}} 
\newcommand{\phibar}{{\bar\phi}} 
\newcommand{\lambar}{{\bar\lambda}} 
\newcommand{\thetabar}{{\bar\theta}} 
\newcommand{\Thetabar}{{\bar\Theta}} 
\newcommand{\betabar}{{\bar\beta}} 
\newcommand{\zetabar}{{\bar\zeta}} 
\newcommand{\etabar}{{\bar\eta}} 
\newcommand{\rhobar}{{\bar\rho}} 
\newcommand{\qbar}{{\bar q}}
\newcommand{\jbar}{{\bar j}}
\newcommand{\Jbar}{{\bar J}}
\newcommand{\Kbar}{{\bar K}}
\newcommand{\Fbar}{{\bar F}}
\newcommand{\Tbar}{{\bar T}}
\newcommand{\cbar}{{\bar c}}
\newcommand{\sbar}{{\bar s}}
\newcommand{\bbar}{{\bar b}}
\newcommand{\Bbar}{{\bar B}}
\newcommand{\ellbar}{{\bar \ell}}

%Hamiltonian and Lagrangians
\newcommand{\Ham}{{\mathcal{H}}}
\newcommand{\Lag}{{\mathcal{L}}}
\newcommand{\Mel}{{\mathcal{M}}}

%Statistical physics
\newcommand{\ZZ}{{\mathcal{Z}}}

\newcommand{\Sp}{{\slashed p}}
\newcommand{\Sq}{{\slashed q}}
\newcommand{\Sk}{{\slashed k}}

%Diagrams
\def\blob[#1]{~\parbox{#1mm}{
\begin{fmfgraph*}(#1,#1)
\fmfleft{i1}
\fmfright{o1}
\fmf{phantom}{i1,v1,o1}
\fmfblob{0.4w}{v1}
\end{fmfgraph*}}~}
\def\vertex[#1]{~\parbox{#1mm}{
  \begin{fmfgraph*}(#1,#1)
    \fmfleft{i1, i2}
    \fmfright{o1,o2}
    \fmf{phantom}{i1,i2,o2,o1,i1}
    \fmf{plain}{i1,v,i2}
    \fmf{plain}{o1,v,o2}
    \fmfforce{nw}{i1}
    \fmfforce{sw}{i2}
    \fmfforce{se}{o1}
    \fmfforce{ne}{o2}
    \fmfforce{c}{v}
    \fmfdot{v}
  \end{fmfgraph*}
  }~}
\def\othervertex[#1]{~\parbox{#1mm}{
  \begin{fmfgraph*}(#1,#1)
    \fmfleft{i1, i2}
    \fmfright{o1,o2}
    \fmf{phantom}{i1,i2,o2,o1,i1}
    \fmf{plain}{i1,v}
    \fmf{plain}{i2,v}
    \fmf{plain}{o1,v}
    \fmf{plain}{v,o2}
    \fmfforce{nw}{i1}
    \fmfforce{sw}{i2}
    \fmfforce{se}{o1}
    \fmfforce{ne}{o2}
    \fmfforce{c}{v}
    \fmfblob{0.3w}{v}
  \end{fmfgraph*}
  }~}
\def\bigvertex[#1]{~\parbox{#1mm}{
  \begin{fmfgraph*}(#1,#1)
    \fmfleft{i1, i2}
    \fmfright{o1,o2}
    \fmf{phantom}{i1,i2,o2,o1,i1}
    \fmf{plain}{i1,v,i2}
    \fmf{plain}{o1,v,o2}
    \fmfforce{nw}{i1}
    \fmfforce{sw}{i2}
    \fmfforce{se}{o1}
    \fmfforce{ne}{o2}
    \fmfforce{c}{v}
    \fmfdot{v}
  \end{fmfgraph*}
  }~}
\def\edge[#1]{~\parbox{#1mm}{
  \begin{fmfgraph*}(#1,#1)
    \fmfleft{i}
    \fmfright{o}
    \fmf{plain,l.s=left}{i,o}
  \end{fmfgraph*}
}~}
\def\curlyedge[#1]{~\parbox{#1mm}{
  \begin{fmfgraph*}(#1,#1)
    \fmfleft{i}
    \fmfright{o}
    \fmf{curly,l.s=left}{i,o}
  \end{fmfgraph*}
}~}
\def\wavyedge[#1]{~\parbox{#1mm}{
  \begin{fmfgraph*}(#1,#1)
    \fmfleft{i}
    \fmfright{o}
    \fmf{wiggly,l.s=left}{i,o}
  \end{fmfgraph*}
}~}
\def\tadpole[#1]{~\parbox{#1mm}{
 	\begin{fmfgraph*}(#1,#1)
 		\fmfleft{i1}
 		\fmfright{o1}
		\fmf{plain}{i1,v1,v1,o1}
 		\fmfdot{v1}
 	\end{fmfgraph*}}~}
\def\amputatedtadpole[#1]{\begin{fmfgraph*}(#1,2)
		\fmfleft{i1}
		\fmfright{o1}
		\fmf{phantom}{i1,v1,o1}
		\fmf{plain}{v1,v1}
		\fmfdot{v1}
	\end{fmfgraph*}}
\def\amputatedwigglytadpole[#1]{\begin{fmfgraph*}(#1,2)
		\fmfleft{i1}
		\fmfright{o1}
		\fmf{phantom}{i1,v1,o1}
		\fmf{wiggly}{v1,v1}
		\fmfdot{v1}
	\end{fmfgraph*}}
\def\amputatedcurlytadpole[#1]{\begin{fmfgraph*}(#1,2)
		\fmfleft{i1}
		\fmfright{o1}
		\fmf{phantom}{i1,v1,o1}
		\fmf{curly}{v1,v1}
		\fmfdot{v1}
	\end{fmfgraph*}}
\def\vacfirstord[#1]{~\parbox{#1mm}{
 	\begin{fmfgraph*}(#1,#1)
		\fmfleft{i1,i2}
		\fmfright{o1,o2}
		\fmf{plain,left}{v2,v1}
		\fmf{plain,left}{v1,v2}
		\fmf{plain,left}{v3,v1}
		\fmf{plain,left}{v1,v3}
		\fmf{phantom}{v2,i1}
		\fmf{phantom}{v3,o1}
		\fmfforce{(0,0)}{i1}
		\fmfforce{(w,0)}{o1}
		\fmfforce{(0.5w,0.5h)}{v1}
		\fmfforce{(0,0.5h)}{v2}
		\fmfforce{(w,0.5h)}{v3}
		\fmfforce{nw}{i2}
		\fmfforce{ne}{o2}
		\fmfforce{(0,0.5h)}{i2}
		\fmfforce{(w,0.5h)}{o2}
		\fmfdot{v1}
		\end{fmfgraph*}}~}
\def\doubletadpolehor[#1]{~\parbox{#1mm}{
\begin{fmfgraph}(#1,#1)
	\fmfleft{i1}
	\fmfright{o1}
	\fmf{plain}{i1,v1,v1,v2,v2,o1}
	\fmfdot{v1,v2}
\end{fmfgraph}
}~}
\def\tripletadpolehor[#1]{~\parbox{#1mm}{
\begin{fmfgraph}(#1,#1)
	\fmfleft{i1}
	\fmfright{o1}
	\fmf{plain}{i1,v1,v1,v2,v2,v3,v3,o1}
	\fmfdot{v1,v2,v3}
\end{fmfgraph}
}~}
\def\doubletadpolever[#1]{~\parbox{#1mm}{
\begin{fmfgraph}(#1,#1)
	\fmfleft{i1}
	\fmfright{o1}
	\fmf{plain}{i1,v1}
	\fmf{plain,left}{v1,v2}
	\fmf{plain,left}{v2,v1}
	\fmf{plain}{v1,o1}
	\fmffreeze
	\fmf{plain,left}{v2,v3,v2}
	\fmfforce{c}{v2}
	\fmfforce{(0.5w,h)}{v3}
	\fmfforce{(0.5w,0)}{v1}
	\fmfforce{sw}{i1}
	\fmfforce{se}{o1}
	\fmfdot{v1,v2}
\end{fmfgraph}
}~}
\def\amputateddoubletadpolever[#1]{~\parbox{#1mm}{
	\begin{fmfgraph}(#1,#1)
	\fmfleft{i1}
	\fmfright{o1}
	\fmf{phantom}{i1,v1}
	\fmf{plain,left}{v1,v2}
	\fmf{plain,left}{v2,v1}
	\fmf{phantom}{v1,o1}
	\fmffreeze
	\fmf{plain,left}{v2,v3,v2}
	\fmfforce{c}{v2}
	\fmfforce{(0.5w,h)}{v3}
	\fmfforce{(0.5w,0)}{v1}
	\fmfforce{sw}{i1}
	\fmfforce{se}{o1}
	\fmfdot{v1,v2}
	\end{fmfgraph}~
}
}
\def\sunset[#1]{\parbox{#1mm}{
\begin{fmfgraph}(#1,#1)
\fmfleft{i}
\fmfright{o}
\fmfforce{0,0.5h}{i}
\fmfforce{w,0.5h}{o}
\fmf{plain,tension=5}{i,v1}
\fmf{plain,tension=5}{v2,o}
\fmf{plain,left,tension=0.5}{v1,v2,v1}
\fmf{plain}{v1,v2}
\fmfdot{v1,v2}
\end{fmfgraph}
}}
\def\amputatedsunset[#1]{\parbox{#1mm}{
\begin{fmfgraph}(#1,#1)
\fmfleft{i}
\fmfright{o}
\fmf{phantom,tension=5}{i,v1}
\fmf{phantom,tension=5}{v2,o}
\fmf{plain,left,tension=0.5}{v1,v2,v1}
\fmf{plain}{v1,v2}
\fmfdot{v1,v2}
\end{fmfgraph}
}}
\def\fourpointsecondorder[#1]{~\parbox{#1mm}{
	\begin{fmfgraph}(15,#1)
	\fmfleft{i1,i2}
	\fmfright{o1,o2}
	\fmf{plain}{i1,v1}
	\fmf{plain}{i2,v1}
	\fmf{plain,right}{v1,v2}
	\fmf{plain,left}{v1,v2}
	\fmf{plain}{v2,o1}
	\fmf{plain}{v2,o2}
	\fmfdot{v1,v2}
	\end{fmfgraph}}~
}
\def\fourpointsecondordertwo[#1]{~\parbox{#1mm}{
	\begin{fmfgraph}(15,#1)
	\fmfleft{i1,i2,i3}
	\fmfright{o1}
	\fmf{plain}{i1,v1}
	\fmf{plain}{i2,v1}
	\fmf{plain}{i3,v1}
	\fmf{plain}{v1,v2,v2,o1}
	\fmfdot{v1,v2}
	\end{fmfgraph}
}~}


\newtheorem{theorem}{Theorem}[section]

\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl(\genfrac..{0pt}{}{#3}{#4} \bigg | #5\biggr)%
        \endgroup
}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{convention}[theorem]{Convention}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{defprop}[theorem]{Definition/Proposition}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\theoremstyle{example}
\newtheorem{example}[theorem]{Example}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{porism}[theorem]{Porism}
\renewcommand\qedsymbol{$\blacksquare$}
\newtheorem{condition}[theorem]{Condition}


